Sub-Goal Trees -- a Framework for Goal-Directed Trajectory Prediction and Optimization

Many AI problems, in robotics and other domains, are goal-directed, essentially seeking a trajectory leading to some goal state. In such problems, the way we choose to represent a trajectory underlies algorithms for trajectory prediction and optimization. Interestingly, most all prior work in imitation and reinforcement learning builds on a sequential trajectory representation -- calculating the next state in the trajectory given its predecessors. We propose a different perspective: a goal-conditioned trajectory can be represented by first selecting an intermediate state between start and goal, partitioning the trajectory into two. Then, recursively, predicting intermediate points on each sub-segment, until a complete trajectory is obtained. We call this representation a sub-goal tree, and building on it, we develop new methods for trajectory prediction, learning, and optimization. We show that in a supervised learning setting, sub-goal trees better account for trajectory variability, and can predict trajectories exponentially faster at test time by leveraging a concurrent computation. Then, for optimization, we derive a new dynamic programming equation for sub-goal trees, and use it to develop new planning and reinforcement learning algorithms. These algorithms, which are not based on the standard Bellman equation, naturally account for hierarchical sub-goal structure in a task. Empirical results on motion planning domains show that the sub-goal tree framework significantly improves both accuracy and prediction time.

==> old_text.tex <==

\section{Formulation - trajectory representations}\label{s:formulation}

and a scalar cost function $c(s,u)$. We are interested in finding a minimum cost path between any two states in the system. Let $V(s,s')$ denote the length of the shortest path from $s$ to $s'$, i.e., 
\begin{equation*}
\begin{split}
    V(s, s') &= \min_{u_0,u_1,\dots,u_T} \sum_{t=0}^{T} c(s_t,u_t) \\
    s.t. &\quad s_0 = s \\
    &\quad s_T = s' \\
    &\quad s_{t+1} = f(s_t, u_t).  
\end{split}
\end{equation*}
We are interested in finding the shortest path. That is, a feasible state sequence from $s$ to $s'$ with accumulated cost $V(s,s')$. We denote this path as $\tau(s,s') = \left\{ s, s_1, s_2, \dots, s' \right\}$
\TJ{after formulation stabilized - add a connector to the next section}




\section{Reinforcement Learning}
We now discuss how to learn $\lambda$ using reinforcement learning. We start from the underlying dynamic programming principle and then proceed to develop learning algorithms.

\subsection{Dynamic Programming Principle}
In this section we derive a dynamic programming principle based on trajectory splitting. 
We consider the all-pairs shortest path problem on a weighted graph, which is a special case of the problem formulation in Section \ref{s:formulation}, in which $c(s,s')$ denotes the weight of edge $s\to s'$. To simplify notation, we replace unconnected edges by edges with weight $\infty$, creating a complete graph. 

Let $V_k(s, s')$ denote the shortest path from $s$ to $s'$ in $2^k$ steps or less. \footnote{note that by our convention about unconnected edges above, if there is no such trajectory in the graph then $V_k(s, s')=\infty$.} We observe the following dynamic programming equation for $V_k$:
\begin{equation}\label{eq:DP_trajsplit}
    \begin{split}
        V_0(s, s') &= c(s, s'), \quad \forall s \neq s'; \\
        V_k(s, s) &= 0, \quad \forall s; \\
        V_k(s, s') &= \min_{s_m} \left\{ V_{k-1}(s, s_m) + V_{k-1}(s_m, s')\right\}, \quad \forall s \neq s'.
    \end{split}
\end{equation}

\begin{theorem}
Consider a weighted graph with $N$ nodes and no negative cycles. Let $V^*(s,s')$ \todo{$V_K^*$ ?} denote the cost of the shortest path from $s$ to $s'$. Let $V_k$ be computed according to \eqref{eq:DP_trajsplit}. For $k \geq \log_2(N)$ we have that $V_k(s, s') = V^*(s, s')$ for all $s,s'$. \todo{how about we split for a thm and col? instead of for $k\ge...$ that we have here, i expected a claim about the relation $V_k$ and shortest path of $k$ steps}
\end{theorem}

\begin{proof}
% \todo{how about proving this by induction?}
We will show by induction that each $V_k(s,s')$ in Algorithm \eqref{eq:DP_trajsplit} is the cost of the shortest path from $s$ to $s'$ in $2^k$ steps or less.

Let $\tau_k(s,s')$ denote a shortest path from $s$ to $s'$ in $2^k$ steps or less, and let $V_k(s,s')$ denote its corresponding cost. 

Our induction hypothesis is that $V_{k-1}(s, s')$ is the cost of the shortest path from $s$ to $s'$ in $2^{k-1}$ steps or less. We will show that $V_k(s, s') = \min_{s_m} \left\{ V_{k-1}(s, s_m) + V_{k-1}(s_m, s')\right\}$.

Assume by contradiction that there was some $s^*$ such that $V_{k-1}(s, s^*) + V_{k-1}(s^*, s') < V_k(s,s')$. Then the concatenated trajectory $[\tau_{k-1}(s,s^*), \tau_{k-1}(s^*,s')]$ would have $2^k$ steps or less, contradicting the fact that $\tau_k(s,s')$ is a shortest path from $s$ to $s'$ in $2^k$ steps or less. So we have that $V_k(s, s') \leq \left\{ V_{k-1}(s, s_m) + V_{k-1}(s_m, s')\right\} \quad \forall s_m$. 

Since the graph is complete, $\tau_k(s,s')$ can be split into two trajectories of length $2^{k-1}$ steps or less. Let $s^{**}$ be a midpoint in such a split. 
Then we have that $V_k(s, s') = \left\{ V_{k-1}(s, s^{**}) + V_{k-1}(s^{**}, s')\right\}$. 

So equality can be obtained and thus we must have $V_k(s, s') = \min_{s_m} \left\{ V_{k-1}(s, s_m) + V_{k-1}(s_m, s')\right\}$.

To complete the induction argument, we need to show that $V_0(s, s') = c(s, s')$. This holds since for $k=0$, for each $s,s'$ there is just one possible trajectory between them of length $1$, which is going through the edge $s,s'$. %Therefore $V_0(s, s') = c(s, s')$.


\todo{should this belongs to the corollary?}
Now, since there are no negative cycles in the graph, for any $s,s'$, the shortest path has at most $N$ steps. Thus, for $k= \log_2 (N)$, we have that  $V_k(s, s')$ is the cost of the shortest path in $N$ steps or less, which is the shortest path between $s$ and $s'$.
\end{proof}

\textbf{Notes:}
\begin{itemize}
    \item The complexity of the algorithm above \todo{todo: write the algorithm explicitly?} is $O(N^3 \log N)$. The Floyd-Warshall algorithm for all-pairs shortest paths is $O(N^3)$, which is similar up to logarithmic factor. However, as we shall see next, our formulation can lead to \emph{learning} based algorithms that use function approximation for the value function.
    \item Note that an $O(N)$ computation is spent on finding the midpoint among all possible nodes. If we can search over a restricted set then there may be a gain there.
    \item I believe that the algorithm will converge even when run asynchronously, i.e., if not all the values from the previous $k$ have finished updating. In this case, several iterations will be required. However, this might be a place to insert a heuristic, as it might be that in many cases we have a good prior on where to look for midpoints in the trajectory. For Euclidean distance, for example, we can start with the Euclidean midpoint, and progressively improve the search, while still using the current estimate for higher values of $k$. 
    \todo{i think you are correct, but it will come at a cost even for the best heuristic:
    we may consider a "message passing" algorithm- when a child at level $K$ is updated, it notifies the parents at level $K+1$ for the change. even if a child at level $K$ finds the minimal on the first try and never updates again, it still needs to send this information to $N^2$ parents, this happens for $N^2$ at every level, and we need $\log{N}$ levels, total of $N^4 \log{N}$ messages.
    compared for messages in sequential algorithm: each parent at level $K$ splits according to a middle state and queries two values: $2N$ messages. this happens for $N^2$ parents with $\log{N}$ levels, total of $N^3 \log{N}$ messages.
    Also the space complexity becomes $N^2 \log{k}$ instead of $2 N^2$
    }
\end{itemize}

\subsection{Reinforcement Learning Algorithms}

We now develop RL algorithms for the Trajectory Split representation based on the dynamic programming algorithm described above. Our main idea is to develop an approximate dynamic programming algorithm for learning $V_k(s, s')$.\todo{f2f comments}

\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{figures/v_k__0.png}
    \includegraphics[width=0.3\textwidth]{figures/v_k__1.png}
    \includegraphics[width=0.3\textwidth]{figures/v_k__2.png}
    \includegraphics[width=0.3\textwidth]{figures/v_k__3.png}
    \includegraphics[width=0.3\textwidth]{figures/v_k__4.png}
    \includegraphics[width=0.3\textwidth]{figures/traj_k_3.png}
    \includegraphics[width=0.3\textwidth]{figures/traj_k_4.png}
    \caption{Approximate DP. Continuous $2$-dimensional particle moving in $8$ directions with an obstacle in the center. Data gathered by random sampling of states and actions. Approximation of $V_k(s, s')$ using K-NN. In (a)-(e) we show the approximate $V_k(s, s'=[0.8,0.8])$ for $k\in[0,\dots,4]$. In (f)-(g) we show the trajectories obtained from $k=3$ and $k=4$.}
    \label{fig:my_label}
\end{figure}

